Physics Opportunities for the Fermilab Booster Replacement

This white paper presents opportunities afforded by the Fermilab Booster Replacement and its various options. Its goal is to inform the design process of the Booster Replacement about the accelerator needs of the various options, allowing the design to be versatile and enable, or leave the door open to, as many options as possible. The physics themes covered by the paper include searches for dark sectors and new opportunities with muons.

==> KDAR.tex <==
\section{Kaons Decay at Rest}

%\textcolor{blue}{Feel free to pick a better title.}

\paragraph{Authors and proponents:} 
%{\textcolor{blue}{
Joshua Spitz, (U. of Michigan)%\footnote{please provide email of corresponding parties in a footnote}. If a collaboration exists, please list it.
%} 

\paragraph{Related sections:}
KDAR may be produced and studied in setups discussed in~\ref{sec:10GeV} and in high energy realizations of the setups in~\ref{sec:1GeV}.

\subsection{Physics Goals, Motivation, and Setup}

\textcolor{blue}{
In this part present a brief description of the physics goals and the motivation. Describe the basics of the setup, the detectors that would be needed, etc. Include references if it is helpful, with bibtex like so~\cite{Alexander:2016aln}. We will use a common \texttt{refs.bib} file. A diagram can be used if it is helpful. If there are nice plots showing the physics impact they can be shown, but are not mandatory. The arrangement should be what you think works best, but please keep the presentation short (of order 1-2 pages for this subsection). If you happen to be writing a letter of intent for a snowmass whitepaper, you can use that text here. A rough draft can be entered initially and can be updated later.  }

\subsection{Accelerator Requirements}

%\textcolor{blue}{
%In this part please provide technical accelerator requirements in the following categories. Feel free to remove categories that do not apply to you or add ones that you think are needed. Its ok to repeat info from the previous subsection here and to include references.  }

\paragraph{Accelerated particles:}
%\textcolor{blue}{
Protons \ldots   %}

\paragraph{Beam Energy:}
%\textcolor{blue}{
$>$2.5~GeV %}

\paragraph{Beam intensity:}
%\textcolor{blue}{
The more protons, the better. The best KDAR source in the world, J-PARC, currently operates at 600~kW. This will upgrade in the next couple of years to 1000~MW. Currently, JSNS$^2$ operates a 17~ton fiducial volume of liquid scintillator neutrino detector at 24~m from this source. So, the Booster replacement and/or associated detector(s) will need to best this in some way in order to be competitive.%}

\paragraph{Beam time structure:}
%\textcolor{blue}{
Pulsed structure with a duty factor $<10^{-3}$ is required to mitigate cosmics. For comparison, the duty factor at J-PARC is $\sim 10^{-5}$.
%}

\paragraph{Target requirements:}
%\textcolor{blue}{
Thick target. Obviously, need strong heat mitigation.%}

\paragraph{Other requirements:}
%\textcolor{blue}{
Lots of shielding for gammas/neutrons between source and detector. Need to think hard about shielding as it relates to detector placement \textit{before} the source or detector are designed.%}

\paragraph{Timescales, R\&D needs, and similar facilities:}
%\textcolor{blue}{
Lots of protons on target and high-power targetry needed. Very similar requirements as the Spallation Neutron Source at ORNL and MLF source at J-PARC, noting that the SNS cannot do KDAR because the energy is too low to produce kaons readily.%}




==> LeptonUniversality.tex <==
\section{Lepton Universality Tests}

\paragraph{Authors and proponents:} 
{\textcolor{blue}{
List of names and affiliations\footnote{please provide email of corresponding parties in a footnote}. If a collaboration exists, please list it.} 

\paragraph{Related sections:}
{\textcolor{blue}{ If there is another menu item which is related to this one, please link to it with a \texttt{ref}.  }


\subsection{Physics Goals, Motivation, and Setup}

\textcolor{blue}{
In this part present a brief description of the physics goals and the motivation. Describe the basics of the setup, the detectors that would be needed, etc. Include references if it is helpful, with bibtex like so~\cite{Alexander:2016aln}. We will use a common \texttt{refs.bib} file. A diagram can be used if it is helpful. If there are nice plots showing the physics impact they can be shown, but are not mandatory. The arrangement should be what you think works best, but please keep the presentation short (of order 1-2 pages for this subsection). If you happen to be writing a letter of intent for a snowmass whitepaper, you can use that text here. A rough draft can be entered initially and can be updated later.  }

\subsection{Accelerator Requirements}

\textcolor{blue}{
In this part please provide technical accelerator requirements in the following categories. Feel free to remove categories that do not apply to you or add ones that you think are needed. Its ok to repeat info from the previous subsection here and to include references.  }

\paragraph{Accelerated particles:}
\textcolor{blue}{
Protons? Electrons? \ldots   }

\paragraph{Beam Energy:}
\textcolor{blue}{
Required energy or energy range and what drives this requirement.  }

\paragraph{Beam intensity:}
\textcolor{blue}{
Required intensity of number of accumulated particles on target to make significant impact.}

\paragraph{Beam time structure:}
\textcolor{blue}{
Pulsed or CW, etc. What is the time structure needed for the physics and what drives these requirments (e.g. reject cosmics, the lifetime of decaying particles, reducing pileup, scaling of backgrounds with instantaneous intensity).  }

\paragraph{Target requirements:}
\textcolor{blue}{
Thin or thick target. Particular element choices. Any other target related relevant info.  }

\paragraph{Other requirements:}
\textcolor{blue}{
Polarization? Need for flexible time structure or beam energy? what else do we need to know? }

\paragraph{Timescales, R\&D needs, and similar facilities:}
\textcolor{blue}{
Is the technology needed to pursue this opportunity ready in the near term? 
List any significant R\&D efforts that would be needed to go forward. Are there facilities in the world, either current or planned, which are would be a precursor to a future Fermilab based experiment or competition to it. References welcome.   }

==> OLD-VERSION-protons-medium-energy.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{amsmath,graphicx}

%\title{ProtonMediumEnergy}
%\author{vdwater }
%\date{June 2020}

% DIMENSION OF TEXT:
%\textwidth 6.0in
%\textheight 8.6in

%\begin{document}

%\maketitle

\section{Fixed-Target Searches for New Physics with $\mathcal{O}$(10 GeV) Proton Beams at Fermi National Accelerator Laboratory}

\bigskip
\paragraph{Contacts: Matt Toups (FNAL) [toups@fnal.gov], R.G. Van de Water (LANL) [vdwater@lanl.gov]}
\medskip

\paragraph{Authors and Proponents: Brian Batell (University of Pittsburg), S.J. Brice (FNAL), Patrick deNiverville (LANL), A. Fava (FNAL), Kevin J. Kelly (FNAL), Tom Kobilarck (FNAL), W.C. Louis (LANL), Pedro A.~N. Machado (FNAL), Bill Pellico (FNAL), Rex Tayloe (Indiana University), R. T. Thornton (LANL),  Z. Pavlovic (FNAL), J. Zettlemoyer (FNAL)}

%{\textcolor{blue}{
%List of names and affiliations\footnote{please provide email of %corresponding parties in a footnote}. If \
%a collaboration exists, please list it.}
%
%\paragraph{Related sections:}
%{\textcolor{blue}{ If there is another menu item which is %related to this one, please link to it with a \\
%texttt{ref}.  }

\subsection{Physics Goals and Motivation}


Proton beam dumps are prolific sources of mesons enabling a powerful technique to search for vector mediator coupling of dark matter to neutral pion and higher mass meson decays.  In the next five years the PIP-II linac will be delivering up to 1 MW of proton power to the FNAL campus.  This includes significant increase of power to the Booster Neutrino Beamline (BNB) which delivers 8 GeV protons to the Short Baseline Neutrino (SBN) detectors.  By building a new dedicated beam dump target station, and using the SBN detectors, a greater than an order of  magnitude increase in search sensitively for dark matter relative to the recent MiniBooNE beam dump search can be achieved.  This modest cost upgrade to the BNB would begin testing models of the highly motivated relic density limit predictions.


Recent theoretical work has highlighted the motivations for
sub-GeV dark matter candidates that interact with ordinary matter
through new light mediator particles \cite{DS}\cite{CVision}\cite{BRN}.
These scenarios constitute a cosmologically and 
phenomenologically viable possibility to account for the dark matter 
of the universe. Such sub-GeV (or light) dark matter particles are difficult to 
probe using traditional methods of dark matter detection, but can be 
copiously produced and then detected with neutrino beam experiments 
such as MiniBooNE, Short Baseline Neutrino (SBN), NOvA, and DUNE \cite{NuDM}.  This represents a new 
experimental approach to search for dark matter and  
is highly complementary to other approaches such as underground direct 
detection experiments, cosmic and gamma ray satellite and balloon 
experiments, neutrino telescopes, and high energy collider 
experiments  \cite{DS}\cite{CVision}\cite{BRN}.  Furthermore, searches for light dark matter provide an 
additional important physics motivation for the current and future 
experimental particle physics research program at the Fermi National Accelerator Laboratory (FNAL).  
%These new ideas are at the core of  DOE/HEP Priority Research Directions 1 call for proposals.
% to 
%fund future small-scale experiments to search
%for dark matter in new and relevant parameter spaces. 
%This proposal leverages the recent novel
%work that has been done at FNAL to directly search for dark matter
%with proton accelerators and neutrino detectors.

The MiniBooNE experiment running at the  FNAL Booster Neutrino Beamline (BNB) was originally designed for neutrino
oscillation and cross section measurements.  In 2014 a special beam dump run was carried out which suppressed neutrino produced backgrounds while enhancing the search for sub-GeV dark matter via neutral current scattering, resulting in new significant sub-GeV dark matter limits \cite{MB-DM}.  The result clearly demonstrated the unique and powerful ability to search for dark matter with a beam dump neutrino experiment.  

\subsection{A New BNB Beam Dump Target Station and Running in the PIP-II Era}

Leveraging the pioneering work of MiniBooNE's dark matter search, it has become clear that a significantly improved sub-GeV dark matter search can be performed with a new dedicated BNB beam dump target station optimized to stop charge pions which produce neutrino backgrounds to a dark matter search.  The new beam dump target can be constructed within 100m of the SBN Near Detector (SBND) that is currently under construction \cite{SBN}. In the PIP-II era 8 GeV protons with higher power can be delivered to the BNB, up to  15 Hz and 115 kW, which is a significant increase from the current 5 Hz and 35 kW. In a five year run this would result in $6\times10^{21}$ Proton on Target (POT) delivered to a new dedicated beam dumped while still delivering maximum levels of protons (35 kW) to the neutrino program. The five year sensitivity would be greater than an order of magnitude better than current MiniBooNE dark matter sensitivity due to the reduced neutrino background from the dedicated beam dump, the detector's close proximity to the beam dump, and higher protons on target.


\begin{figure}[ht]
 \centerline{ 
 \includegraphics[width=0.45\textwidth]{SBND_Inelastic_Nucleon.pdf}\hspace*{0.3cm}
 \includegraphics[width=0.45\textwidth]{SBND_electron.pdf}\hspace*{0.3cm}
 }
\caption{\footnotesize Regions of relic abundance parameter (mixing
  strength) $Y$ vs. dark matter mass $m_\chi$ for $6\times10^{21}$ POT that could be
  achieved in a five year run with dedicated proton beam dump medium energy running in the PIP-II era. Left is the signal sensitivity for NC$\pi^0$ and right for NC-electron scattering with the SBND detector at 100 m from the dedicated beam dump.  Both panels show regions where we expect 1--10 (light green), 10--1000 (green), and more than 1000 (dark green) scattering events. The solid black line is the scalar relic density line that can be probed.}
\label{ExpSensitivity1}
\end{figure}




\subsubsection{Required Infrastructure}
The new PIP-II linac will be able to deliver a proton beam of significantly higher-power to the Booster than the current linac. This will result in 15 Hz of beam to be delivered to the BNB achieving 115 kW, or about three times the power of current delivery.   The BNB neutrino target and horn have a power limit of 35 kW, which leaves 80 kW of power for other uses. A new target station fed by the BNB, and on axis with the existing SBN neutrino experiment could be built relatively quick and at modest cost.  Such a facility could be run concurrently with the SBN neutrino program, only using protons beyond the 35 kW limit.  Events would be trivially separated on a pulse by pulse basis based on the which target the beam is being delivered too. The facility will require a Fe target about 2 m in length and 1 m in width to absorb the protons and resulting charged pions.  Shielding and cooling requirements up to 80 kW are straightforward.  Such a target would reduce the neutrino backgrounds by another three orders of magnitude relative the regular neutrino running (see next section for details).  Besides the higher power, the reduced neutrino flux background enables a significantly more sensitive search for dark matter relative to the MiniBooNE beam off target run.

\subsubsection{Neutrino Flux Reduction with Improved Beam Dump}

To leverage the increased signal rate production, a
corresponding reduction in neutrino-induced backgrounds is required.
The MiniBooNE-DM beam-off-target run steered the protons past the Be
target/horn and onto the 50 m absorber.  This reduces the
neutrino-induced background rate by a factor of $\sim$50, but there
was still significant production of neutrinos from proton interactions
in the 50 m of decay pipe air and beam halo scraping of the target.
Further reduction of neutrino production occurs by directing the proton beam directly onto a 
dense beam stop absorber made of Fe or W.  This puts the end of
the proton beam pipe directly onto the dump with no air gap.  Detailed BNB dump beam line simulations, which have been verified by data \cite{MB-DM}, demonstrate that this would reduce
neutrino-induced backgrounds by a factor of 1000 over Be-target neutrino
running, which is a factor of twenty better than the 50 m
absorber as demonstrated in Figure \ref{NuFlux}.  

\begin{figure}[h]
 \centerline{ 
 \includegraphics[width=0.5\textwidth]{ccqe_steel_target_compare.eps}\hspace*{0.3cm}}
\caption{\footnotesize Detailed neutrino flux estimation for neutrino running 
  (solid black line), beam-off-target 50 m absorber running (dotted red line), 
  and a dedicated new BNB beam dump target station (dotted brown line).   In this final mode, the neutrino 
  flux reduction is a factor of 1000, or about 20 times better than 
  50 m absorber running. }
\label{NuFlux}
\end{figure}



\subsection{Accelerator Requirements}

Require a new dedicated beam dump either reusing the the BNB or a separate new beam line.   The best and cheapest option is to build a dedicated dump feed by the BNB (kicker magnet just upstream of the current neutrino target/horn) and 100 m from the SBND detector.  

\paragraph{Accelerated particles:}
%\textcolor{blue}{Protons? Electrons? \ldots   }
Protons

\paragraph{Beam Energy:}
%\textcolor{blue}{Required energy or energy range and what drives this requirement.  }
On order of 10 GeV.  Sensitivity studies have been performed for 8 GeV BNB line, but slightly lower and higher energies would have similar sensitivities.  

\paragraph{Beam intensity:}
%\textcolor{blue}{
%Required intensity of number of accumulated particles on target %to make significant impact.}

Currently the BNB runs 35 kW maximum do to constraints on the horn and target.  Having a separate beam dump target station would allow higher beam power, with up to 115 kW, limited by radiation beamline losses and target cooling requirements.

\paragraph{Beam time structure:}

Beam spills less than a few usec with separation between spills greater than 50 usec.  Shorter beam spills reduce cosmogenic and other random backgrounds. RF structure on the scale of $\sim$1 nsec enable dark matter time of flight measurements increasing sensitivity. Requires detectors with similar timing capability.

\paragraph{Target requirements:}

Thick ($\sim$meters) dense targets (Fe, W, U, etc) are ideal for ranging out charged pions and stopping them before decaying into neutrinos, which form the biggest background for beam dark matter searches.    
%\textcolor{blue}{
%Thin or thick target. Particular element choices. Any other %target related relevant info.  }

\paragraph{Other requirements:}
%\textcolor{blue}{
%Polarization? Need for flexible time structure or beam energy? %what else do we need to know? }
Building a dedicated beam dump and maintaining the current neutrino target allow flexible physics goals (sterile neutrinos and dark sector searches), maximum use of POT, and utilization of shared resources like the BNB beam line.

\paragraph{Timescales, R\&D needs, and similar facilities:}
%\textcolor{blue}{
%Is the technology needed to pursue this opportunity ready in the near term?
%List any significant R\&D efforts that would be needed to go forward. Are there %facilities in the world, \
%either current or planned, which are would be a precursor to a future Fermilab based %experiment or compet\
%ition to it. References welcome.   }


The timescale is similar to the construction of PIP-II and the expected upgrade in protons once online. The SBN detectors are expected to run for at least 10 years. The new dedicated beam dump could be built sooner and begin running using the SBN detectors at a lower rate until the PIP-II upgrade is complete. Such a facility could be built quickly, 1-2 years, and at modest cost below \$5M.  There are no other similar facilities in the world currently or planned in the next five years that can probe for dark matter masses up to 1 GeV with a proton beam.

\begin{thebibliography}{}

\bibitem{DS} "Dark Sectors 2016 Workshop: Community Report", arXiv:1608.08632",  2016

\bibitem{CVision} Battaglieri {\it et al.}, "US Cosmic Visions: New Ideas in Dark Matter 2017: Community Report", arXiv:1707.04591", FERMILAB-CONF-17-282-AE-PPD-T", 2017.

\bibitem{BRN} "Basic Research Needs For Dark Matter Small Projects New Initiatives'',
https://science.osti.gov/-/media/hep/pdf/Reports/Dark\_Matter\_New\_Initiatives\_rpt.pdf, 2018

\bibitem{NuDM} P.\ deNiverville, M.\ Pospelov, A.\ Ritz", "Observing a light dark matter beam with neutrino experiments", Phys.Rev. D84", 075020", arXiv: 1107.4580, 2011.


\bibitem{MB-DM} 
  A.~A.~Aguilar-Arevalo {\it et al.} [MiniBooNE DM Collaboration],
  ``Dark Matter Search in Nucleon, Pion, and Electron Channels from a Proton Beam Dump with MiniBooNE,''
  Phys.\ Rev.\ D {\bf 98}, no. 11, 112004 (2018)
  %doi:10.1103/PhysRevD.98.112004
  [arXiv:1807.06137 [hep-ex]].
  
\bibitem{SBN}
P.~A.~Machado, O.~Palamara and D.~W.~Schmitz,
%``The Short-Baseline Neutrino Program at Fermilab,''
Ann. Rev. Nucl. Part. Sci. \textbf{69}, 363-387 (2019)
doi:10.1146/annurev-nucl-101917-020949
[arXiv:1903.04608 [hep-ex]].
%24 citations counted in INSPIRE as of 28 Aug 2020

\end{thebibliography}

%\end{document}


==> electron-nucleus.tex <==
\section{Electron-Nucleus Scattering}
**** NOTE HAS BEEN MOVED TO lepton-nucleon.tex ***
\paragraph{Authors and proponents:} 
{\textcolor{blue}{
List of names and affiliations\footnote{please provide email of corresponding parties in a footnote}. If a collaboration exists, please list it.} 

\paragraph{Related sections:}
{\textcolor{blue}{ If there is another menu item which is related to this one, please link to it with a \texttt{ref}.  }


\subsection{Physics Goals, Motivation, and Setup}

\textcolor{blue}{
In this part present a brief description of the physics goals and the motivation. Describe the basics of the setup, the detectors that would be needed, etc. Include references if it is helpful, with bibtex like so~\cite{Alexander:2016aln}. We will use a common \texttt{refs.bib} file. A diagram can be used if it is helpful. If there are nice plots showing the physics impact they can be shown, but are not mandatory. The arrangement should be what you think works best, but please keep the presentation short (of order 1-2 pages for this subsection). If you happen to be writing a letter of intent for a snowmass whitepaper, you can use that text here. A rough draft can be entered initially and can be updated later.  }

\subsection{Accelerator Requirements}

\textcolor{blue}{
In this part please provide technical accelerator requirements in the following categories. Feel free to remove categories that do not apply to you or add ones that you think are needed. Its ok to repeat info from the previous subsection here and to include references.  }

\paragraph{Accelerated particles:}
\textcolor{blue}{
Protons? Electrons? \ldots   }

\paragraph{Beam Energy:}
\textcolor{blue}{
Required energy or energy range and what drives this requirement.  }

\paragraph{Beam intensity:}
\textcolor{blue}{
Required intensity of number of accumulated particles on target to make significant impact.}

\paragraph{Beam time structure:}
\textcolor{blue}{
Pulsed or CW, etc. What is the time structure needed for the physics and what drives these requirments (e.g. reject cosmics, the lifetime of decaying particles, reducing pileup, scaling of backgrounds with instantaneous intensity).  }

\paragraph{Target requirements:}
\textcolor{blue}{
Thin or thick target. Particular element choices. Any other target related relevant info.  }

\paragraph{Other requirements:}
\textcolor{blue}{
Polarization? Need for flexible time structure or beam energy? what else do we need to know? }

\paragraph{Timescales, R\&D needs, and similar facilities:}
\textcolor{blue}{
Is the technology needed to pursue this opportunity ready in the near term? 
List any significant R\&D efforts that would be needed to go forward. Are there facilities in the world, either current or planned, which are would be a precursor to a future Fermilab based experiment or competition to it. References welcome.   }

==> medium-energy.tex <==

\section{Dark Matter Search with Intermediate Energy Protons}
\label{sec:proton-beam-dumps}

\paragraph{Authors and proponents:
R.G. Van de Water (LANL), Matt Toups (FNAL), Tom Kobilarck (FNAL), et. al.}

%{\textcolor{blue}{
%List of names and affiliations\footnote{please provide email of %corresponding parties in a footnote}. If \
%a collaboration exists, please list it.}
%
%\paragraph{Related sections:}
%{\textcolor{blue}{ If there is another menu item which is %related to this one, please link to it with a \\
%texttt{ref}.  }

\subsection{Physics Goals, Motivation, and Setup}

%\textcolor{blue}{
%In this part present a brief description of the physics goals %and the motivation. Describe the basics of \
%the setup, the detectors that would be needed, etc. Include %references if it is helpful, with bibtex like\
% so~\cite{Alexander:2016aln}. We will use a common %\texttt{refs.bib} file. A diagram can be used if it is\
%5 helpful. If there are nice plots showing the physics impact %they can be shown, but are not mandatory. Th\
%e arrangement should be what you think works best, but please %keep the presentation short (of order 1-2 p\
%ages for this subsection). If you happen to be writing a letter %of intent for a snowmass whitepaper, you \
%can use that text here. A rough draft can be entered initially %and can be updated later.  }

Recent theoretical work has highlighted the motivations for
sub-GeV dark matter candidates that interact with ordinary matter
through new light mediator particles.
These scenarios constitute a cosmologically and 
phenomenologically viable possibility to account for the dark matter 
of the universe. Such sub-GeV (or light) dark matter particles are difficult to 
probe using traditional methods of dark matter detection, but can be 
copiously produced and then detected with neutrino beam experiments 
such as MiniBooNE, Short Baseline Neutrino (SBN), NOvA, and DUNE.  This represents a new 
experimental approach to search for dark matter and  
is highly complementary to other approaches such as underground direct 
detection experiments, cosmic and gamma ray satellite and balloon 
experiments, neutrino telescopes, and high energy collider 
experiments.  This has been highlighted recently in the
``U.S. Cosmic Visions: New Ideas in Dark Matter 2017:
Community Report'' white paper. Furthermore, searches for light dark matter provide an 
additional important physics motivation for the current and future 
experimental particle physics research program at the Fermi National Accelerator Laboratory (FNAL).  
%These new ideas are at the core of  DOE/HEP Priority Research Directions 1 call for proposals.
% to 
%fund future small-scale experiments to search
%for dark matter in new and relevant parameter spaces. 
%This proposal leverages the recent novel
%work that has been done at FNAL to directly search for dark matter
%with proton accelerators and neutrino detectors.

The MiniBooNE experiment running at the  FNAL Booster Neutrino Beamline (BNB) was originally designed for neutrino
oscillation and cross section measurements, and completed this program in 2012.  In 2014 a special beam dump run was carried out which suppressed neutrino produced backgrounds while enhancing the search for sub-GeV dark matter via neutral current scattering, resulting in new significant sub-GeV dark matter limits (citation).  The result clearly demonstrated the unique and powerful ability to search for dark matter with a beam dump neutrino experiment.  
It has become clear that up to $\sim$1 orders of magnitude improved sub-GeV dark matter search can be performed with a new dedicated BNB beam dump constructed within 100m either the SBND near detector, or a new large (kton) and fast (nsec) detector similar in performance to the MiniBooNE detector. Coupled with  higher powered protons delivered by PIP-II (15 Hz at 115 kW) to the BNB, the sensitivity
after a five year run would be more than 1-2 orders of magnitude better than current MiniBooNE dark matter sensitivity due to the reduced neutrino background from the upgraded beam dump, the detector's close proximity to the beam dump, and higher protons on target.  
The improved sensitivity will test many models of the highly motivated relic density limit predictions.  
%This proposal outlines an extensive sub-GeV dark matter search addressing PRD 1, done as a Track 1 two year program for a \$1.1M total budget, and includes the design of a dedicated beam dump, %schedule, and performance estimates

\begin{figure}[ht]
 \centerline{ 
 \includegraphics[width=0.5\textwidth]{SBND_10E20_Inelastic_Pion.pdf}\hspace*{0.3cm}
 \includegraphics[width=0.5\textwidth]{SBND_10E20_NCE_Electron.pdf}\hspace*{0.3cm}
 }
\caption{\footnotesize Regions of relic abundance parameter (mixing
  strength) $Y$ vs. dark matter mass $m_\chi$ for $10\times10^{20}$ POT that could be
  achieved  with dedicated proton beam dump medium energy running in the PIP-II era. Left is the signal sensitivity for NC$\pi^0$ and right for NC-electron scattering with the SBND detector at 100 m from the dump.  Both panels show regions where we expect 1--10 (light green), 10--1000 (green), and more than 1000 (dark green) scattering events. {\bf Need to update plot }}
\label{ExpSensitivity1}
\end{figure}




\subsection{Accelerator Requirements}

Require a new dedicated beam dump either reusing the the BNB or a separate new beam line.   One option is to build a dedicated dump parallel to the current neutrino target/horn. The SBND near detector can then be re-used to make measurements.  To further increase the sensitivity, a MiniBooNE-like - 1 kton fast Cerenkov - detector could be built at 100 m from the target.
A dedicated near beam dump with higher powered protons delivered to BNB from PIP-II will result in 1-2 orders of magnitude improved DM sensitivity from what was measured by MiniBooNE.
%\textcolor{blue}{
%In this part please provide technical accelerator requirements in %the following categories. Feel free to \
%remove categories that do not apply to you or add ones that you %think are needed. Its ok to repeat info f\
%rom the previous subsection here and to include references.  }

\paragraph{Accelerated particles:}
%\textcolor{blue}{Protons? Electrons? \ldots   }
Protons

\paragraph{Beam Energy:}
%\textcolor{blue}{Required energy or energy range and what drives this requirement.  }
On order of 10 GeV.  Sensitivity studies have been performed for 8 GeV BNB line, but slightly lower and higher energies would have similar sensitivities.  

\paragraph{Beam intensity:}
%\textcolor{blue}{
%Required intensity of number of accumulated particles on target %to make significant impact.}

Currently the BNB runs 35 kW maximum do to constraints on the horn and target.  Having a separate beam dump target station would allow higher beam power, with up to 115 kWatts, limited by radiation beamline losses and target cooling requirements.

\paragraph{Beam time structure:}
%\textcolor{blue}{
%Pulsed or CW, etc. What is the time structure needed for the %physics and what drives these requirments (e\
%.g. reject cosmics, the lifetime of decaying particles, reducing %pileup, scaling of backgrounds with inst\
%antaneous intensity).  }

Beam spills less than a few usec with separation between spills greater than 50 usec.  Shorter beam spills reduce cosmogenic and other random backgrounds. RF structure on the scale of ~1 nsec enable dark matter time of flight measurements increasing sensitivity. Requires detectors with similar timing capability.

\paragraph{Target requirements:}

Thick (few meters) dense targets (Fe, W, U, etc) are ideal for ranging out charged pions and stopping them before decaying into neutrinos, which form the biggest background for beam dark matter searches.    
%\textcolor{blue}{
%Thin or thick target. Particular element choices. Any other %target related relevant info.  }

\paragraph{Other requirements:}
%\textcolor{blue}{
%Polarization? Need for flexible time structure or beam energy? %what else do we need to know? }
Building a dedicated beam dump and separate neutrino target allow flexible physics goals, maximum use of POT, and utilization of shared resources like the BNB beam line.

\paragraph{Timescales, R\&D needs, and similar facilities:}
%\textcolor{blue}{
%Is the technology needed to pursue this opportunity ready in the near term?
%List any significant R\&D efforts that would be needed to go forward. Are there %facilities in the world, \
%either current or planned, which are would be a precursor to a future Fermilab based %experiment or compet\
%ition to it. References welcome.   }

Timescale is similar to construction of PIP-II and the expected upgrade in protons once online.  The dedicated beam dump will be built during this time frame.





==> proton-irradiation_copy.tex <==
\section{Proton Irradiation Facility}% Petra Merkel

\paragraph{Authors and proponents:} 
{\textcolor{blue}{
Maral Alyari, Artur Apresyan, Doug Berry, Zoltan Gecse, Mandy Kiburg, Thomas Kobilarcik, Ron Lipton, Petra Merkel, Evan Niner, Eduard Pozdeyev, all Fermilab  \footnote{corresponding author: petra@fnal.gov}} 

\paragraph{Related sections:}
{\textcolor{blue}{ Should link to new testbeam proposal when ready... \texttt{ref}.  }


\subsection{Physics Goals, Motivation, and Setup}

\textcolor{blue}{
The goal is to create a high-intensity proton irradiation facility at the Fermilab Booster Replacement to benefit future collider detector development. The current Fermilab Irradiation Test Area (ITA), which is under construction right now at the end of the LINAC, is designed for fluences needed for the HL-LHC detector upgrades. However, for future collider detectors doses up to two orders of magnitude higher are expected. It is paramount that detector elements under development can be tested for radiation hardness to these levels. Currently, there is no facility in the world, that would allow such tests at a reasonable timescale. It would be desirable to reach on the order of 10$^{18}$ protons within a few hours. The exact beam energy is less critical. The DOE program manager for detectors has expressed interest in Fermilab creating such a facility. The Fermilab Booster Replacement seems like an ideal candidate with its high intensity proton beam. The proposal is to build a tangential arm to set up an experimental hall where devices under test can be placed for irradiation under controlled conditions. }

\subsection{Accelerator Requirements}

\textcolor{blue}{
It would be desirable to reach on the order of 10$^{18}$ protons within a few hours. The exact beam energy is less critical. The beamsize at the device under test (DUT) should be on the order of a few millimeters to two centimeters. A pulsed beam would be preferable for cooling and readout reasons.  }

\paragraph{Accelerated particles:}
\textcolor{blue}{
The main particle type that is needed would be protons, but being able to switch to electrons, or even ions at times, would be beneficial. }

\paragraph{Beam Energy:}
\textcolor{blue}{
We would take the maximum achievable beam energy. The absolute value is not so relevant, as long as it is stable and known.  }

\paragraph{Beam intensity:}
\textcolor{blue}{
It would be desirable to reach on the order of 10$^{18}$ protons within a few hours.}

\paragraph{Beam time structure:}
\textcolor{blue}{
A pulsed beam would be preferable, or even necessary. A continuous beam would likely overheat the DUT and make cooling very challenging. Even with a pulsed beam, cooling of the DUT will be one of the main challenges. A similar time structure to the current LINAC could be suitable.}

\paragraph{Target requirements:}
\textcolor{blue}{
No target is needed. We would need a stripping station to strip off the electrons from the beam, but the target would be the user provided DUTs. }

\paragraph{Other requirements:}
\textcolor{blue}{
It would be good to have an adjacent, shielded counting room, where users could sit and operate and monitor their DUTs. This would also require some user infrastructure, such as cables, power supplies, cooling, to be placed either in the experimental hall or the adjacent counting room. Cables would need to run between the two. There should be a cold, dark box for the DUTs available that can be moved in and out of the beam, including beam scans. Beam monitoring data need to be made available to the users as well. The irradiated DUTs would be handled by rad techs. and stored cold until they can be retrieved by the users.}

\paragraph{Timescales, R\&D needs, and similar facilities:}
\textcolor{blue}{
Likely, cooling of the DUTs is the main challenge and some R\&D needs to go into finding a solution for this. Similarly, having robotic control of handling the box that contains the DUTs and that needs to move in and out of the beam would be highly desirable. This could be either addressed by a commercial solution or by in-house development. The timescale by which such a facility is needed would realistically be somewhere in the second half of the 2020s. Before then, detector components aimed to sustain these kinds of radiation levels will likely not be ready for testing.  }



